Robust Fingerprinting of Genomic Databases

Database fingerprinting has been widely used to discourage unauthorized redistribution of data by providing means to identify the source of data leakages. However, there is no fingerprinting scheme aiming at achieving liability guarantees when sharing genomic databases. Thus, we are motivated to fill in this gap by devising a vanilla fingerprinting scheme specifically for genomic databases. Moreover, since malicious genomic database recipients may compromise the embedded fingerprint by launching effective correlation attacks which leverage the intrinsic correlations among genomic data (e.g., Mendel's law and linkage disequilibrium), we also augment the vanilla scheme by developing mitigation techniques to achieve robust fingerprinting of genomic databases against correlation attacks. We first show that correlation attacks against fingerprinting schemes for genomic databases are very powerful. In particular, the correlation attacks can distort more than half of the fingerprint bits by causing a small utility loss (e.g.,database accuracy and consistency of SNP-phenotype associations measured via p-values). Next, we experimentally show that the correlation attacks can be effectively mitigated by our proposed mitigation techniques. We validate that the attacker can hardly compromise a large portion of the fingerprint bits even if it pays a higher cost in terms of degradation of the database utility. For example, with around 24% loss in accuracy and 20% loss in the consistency of SNP-phenotype associations, the attacker can only distort about 30% fingerprint bits, which is insufficient for it to avoid being accused. We also show that the proposed mitigation techniques also preserve the utility of the shared genomic databases.

==> sections/preliminaries.tex <==
%\section{Preliminaries}

\section{The Vanilla Fingerprint Scheme}
\label{sec:vanilla}

In this work, we consider the  fingerprinting scheme proposed in \cite{li2005fingerprinting} as the vanilla scheme, for which we show the vulnerability and develop the proposed scheme.  
% This scheme It extends the watermarking  scheme developed in \cite{agrawal2003watermarking} in a significant way to
% supports the insertion and detection of arbitrary fingerprint bit-string  in databases.  
Assume a database owner shares her data with multiple service providers (SPs). The fingerprint  of a specific SP is obtained using a cryptographic hash function, whose input is the concatenation of the database owner's secret key and the SP's public series number. For fingerprint insertion, the vanilla scheme  pseudorandomly selects one bit position of one attribute of some data records in the database and replaces those bits with the results obtained from the exclusive or (XOR) between mask bits and fingerprint bits, both of which are also determined pseudorandomly.  
For fingerprint extraction, the scheme locates the exact positions of the potentially changed bits,   calculates the fingerprint bits by XORing those bits with the exact mask bits, and finally recovers each bit in the  fingerprint bit-string via majority voting, since each fingerprint bit can be  used to mark many different positions.
% \footnote{Please refer to Figure 1 on page 36 and Figure 2 on page 37 in \cite{li2005fingerprinting} for the pseudocodes of fingerprint insertion and extraction of the considered vanilla scheme.} 
To preserve the utility of the fingerprinted database, we will let the vanilla scheme only change the least significant bit (LSB) of selected database entries. {\color{black}For completeness, in Appendix \ref{sec:vanilla-steps}, we show the steps to insert fingerprint into a database, and the steps to extract fingerprint from a pirated   database, in Algorithms \ref{algo:vanilla-insert} and \ref{algo:vanilla-extract}, respectively.} In Appendix \ref{sec:utility_LSB},  we empirically  validate  that only changing the LSB indeed leads to higher utility than altering one of the least $k$ significant bits (L$k$SB) of selected entries. 


In practice, one can choose any database fingerprinting scheme as the vanilla scheme, because our proposed mitigation techniques are independent of the adopted vanilla scheme, and they can be used as post-processing steps on top of any existing database fingerprinting schemes. 
The reason we choose the aforementioned  vanilla scheme  is because
% (i) it is a key-based scheme, which uses secret key in each step of the fingerprint insertion and detection, (ii) it does not require storing all the SP-fingerprint pairs in another database for detection purpose, (iii) it processes each data record independently, 
(i) it is shown to have high robustness, e.g., the probability of detecting no fingerprint as a result of random bit flipping attack (a common attack against fingerprinting schemes, as will be discussed in Section~\ref{sec:threat_models}) is upper bounded by ${(|SP|-1)}/{2^L}$, where $|SP|$ is the number of SPs who have received the fingerprinted copies and $L$ is the length of the fingerprint bit-string, (ii) it is shown to be robust even if some fingerprinted entries are identified by a malicious SP, because it applies majority voting on all the fingerprinted entries to extract the fingerprint bit-string, 
and (iii) it can easily be extended to incorporate Boneh-Shaw code \cite{boneh1998collusion} to defend against collusion attacks.  {\color{black}Our developed  robust fingerprinting scheme inherits all the properties of the vanilla  scheme because (i) it uses the  vanilla scheme as the building block and (ii) it does not alter the entries that have already been changed by the vanilla scheme (due to fingerprinting insertion).}


